Cell-ontology guided transcriptome foundation model

Transcriptome foundation models TFMs hold great promises of deciphering the transcriptomic language that dictate diverse cell functions by self-supervised learning on large-scale single-cell gene expression data, and ultimately unraveling the complex mechanisms of human diseases. However, current TFMs treat cells as independent samples and ignore the taxonomic relationships between cell types, which are available in cell ontology graphs. We argue that effectively leveraging this ontology information during the TFM pre-training can improve learning biologically meaningful gene co-expression patterns while preserving TFM as a general purpose foundation model for downstream zero-shot and fine-tuning tasks. To this end, we present single cell, Cell-ontology guided TFM scCello. We introduce cell-type coherence loss and ontology alignment loss, which are minimized along with the masked gene expression prediction loss during the pre-training. The novel loss component guide scCello to learn the cell-type-specific representation and the structural relation between cell types from the cell ontology graph, respectively. We pre-trained scCello on 22 million cells from CellxGene database leveraging their cell-type labels mapped to the cell ontology graph from Open Biological and Biomedical Ontology Foundry. Our TFM demonstrates competitive generalization and transferability performance over the existing TFMs on biologically important tasks including identifying novel cell types of unseen cells, prediction of cell-type-specific marker genes, and cancer drug responses.

==> sections/03_perliminary.tex <==
%\vspace{-0.5em}
\section{Preliminary}
\label{sec:preliminary}













==> sections/figure_tex/_cell_type_classification_and_CDR_prediction.tex <==
\begin{table}[t]
    \begin{minipage}[t]{0.69\textwidth}
        \centering
        \caption{\textbf{Cell Type Classification} on In-distribution Data ($D^{id}$). After fine-tuning, we report classification results and compare clustering performance between the fine-tuned and zero-shot TFMs.}
        %\label{tab:standard_cell_type_classification}
        \begin{adjustbox}{max width=\textwidth}
            \begin{tabular}{l|cc|cc|c}
            \toprule
            \multirow{2}{*}{\bf{Method}} & \multicolumn{2}{c|}{Classification} & \multicolumn{3}{c}{Clustering (AvgBio $\uparrow$)} \\
    
            \cmidrule{2-3} \cmidrule{4-6}
            & Acc $\uparrow$ & Macro F1 $\uparrow$ & Fine-tuned & Zero-shot &  $\Delta_{\mathrm{AvgBio}} \uparrow$ \\
            
            \midrule
            \multicolumn{6}{c}{\bf{Training from Scratch for \method}} \\
            \midrule
            \methodscratch & 0.621 & 0.223 & 0.544 & / & / \\
            
            
            \midrule
            \multicolumn{6}{c}{\bf{Ontology-Agnostic TFMs}} \\
            \midrule
    
            Geneformer & 0.747 & 0.440& 0.439 & 0.432 & +0.007 \\
            

    scGPT & 0.712 & 0.344 & 0.477 & 0.438 & +0.039 \\
    scTab & 0.778 & 0.373 & 0.606 & \underline{0.577} & +0.029 \\
    \mgprepro & 0.722 & 0.287 & 0.607  & 0.473   & +0.134 \\
    \suprepro & 0.812 & 0.363 & \underline{0.659}  & 0.555 & +0.104 \\
    \mgpsuprepro & \underline{0.820} & \underline{0.406} & 0.607  & 0.516 & +0.091 \\
    
            \midrule
            \multicolumn{6}{c}{\bf{Ontology-Enhanced TFMs}} \\
            \midrule
    
            \method & \bf{0.867} & \bf{0.511} & \bf{0.694}  & \bf{0.670} & +0.024 \\
            
            \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.28\textwidth}
        % NOTE: fill scTab
        \centering
        \captionof{table}{\textbf{Cancer Drug\qquad Response Prediction} for \quad regression of $IC_{50}$ values}
        %\label{tab:exp_cancer_drug_response_prediction}
        %\footnotesize
        \begin{adjustbox}{max width=\textwidth, max height=0.743\textwidth}
            \begin{tabular}{l|c}
                \toprule
                Method & PCC$\uparrow$ \\

                \midrule
                \multicolumn{2}{c}{\bf{Non-TFM Methods}} \\
                \midrule
                DeepCDR	& 0.854 \\

                \midrule
                \multicolumn{2}{c}{\bf{Ontology-Agnostic TFMs}} \\
                \midrule
                scFoundation & 0.882 \\
                Geneformer & 0.911 \\
                scGPT & \textbf{0.919} \\
                scTab & 0.913 \\
                UCE & \textbf{0.922} \\
                \mgprepro & 0.872 \\
                \suprepro & 0.915 \\
                \mgpsuprepro & \underline{0.916} \\
            
                \midrule
                \multicolumn{2}{c}{\bf{Ontology-Enhanced TFMs}} \\
                \midrule

                \method & \textbf{0.917} \\
    
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{minipage}
    \vspace{-0.5cm}
\end{table}


\begin{table}[t]
    \begin{minipage}[t]{0.56\textwidth}
        \centering
        \caption{\textbf{Cell Type Classification}. After fine-tuning, we report the classification and clustering results, and the clustering improvement against that before fine-tuning.}
        \label{tab:standard_cell_type_classification}
        \begin{adjustbox}{max width=\textwidth}
            \begin{tabular}{l|cc|cc}
            \toprule
            \multirow{2}{*}{\bf{Method}} & \multicolumn{4}{c}{$D^{id}$}\\

            \cmidrule{2-3} \cmidrule{4-5}
            & Acc $\uparrow$ & Macro F1 $\uparrow$ & AvgBio $\uparrow$ & $\Delta_{\mathrm{AvgBio}} \uparrow$  \\ 

            %\midrule
            %\multicolumn{5}{c}{\bf{Training from Scratch for Fine-tuning Tasks}} \\
            \midrule
            \methodscratch & 0.621 & 0.223 & 0.544 &  /  \\
            
            \midrule
            \multicolumn{5}{c}{\methodheadlinetfmbsl} \\
            \midrule
    
            Geneformer & 0.747 & 0.440& 0.439 & +0.007   \\
            

    scGPT & 0.712 & 0.344 & 0.477 &  +0.039  \\
    scTab & 0.778 & 0.373 & 0.606 &  +0.029  \\
    \mgprepro & 0.722 & 0.287 & 0.607  & +0.134 \\
    \suprepro & 0.812 & 0.363 & \underline{0.659}  & +0.104  \\
    \mgpsuprepro & \underline{0.820} & \underline{0.406} & 0.607  &  +0.091   \\
    
            \midrule
            \multicolumn{5}{c}{\methodheadlineourtfm} \\
            \midrule
    
            \method & \bf{0.867} & \bf{0.511} & \bf{0.694}  & +0.024 \\
            \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{minipage}

\end{table}

==> sections/figure_tex/_cell_type_identification.tex <==


\iffalse
\begin{table}[t]
    \begin{minipage}[t]{0.41\textwidth}
    
    \centering
    \caption{In-distribution Zero-shot Clustering. Four metrics are reported for completeness.}
    % \label{tab:indist_cell_type_clustering}
    %\footnotesize
    \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{l|ccc|c}
        \toprule
        \multirow{2}{*}{\bf{Method}} & \multicolumn{4}{c}{ID Unseen Data ($D^{id}$)}\\
        
        \cmidrule{2-5}
        & NMI$_{c}$$\uparrow$ & ARI${_c}$$\uparrow$ & ASW${_c}$$\uparrow$ & \bf{AvgBio}$\uparrow$\\
        
        \midrule
        \multicolumn{5}{c}{\bf{Traditional Methods \emph{w/o} Pre-training}} \\
        \midrule
        
        Raw Data & 0.566 & 0.237 & 0.453 & 0.419 \\
        Seurat & 0.648 & 0.270 & 0.407 & 0.442 \\
        Harmoney & 0.621 & 0.261 & 0.382 & 0.421 \\
        scVI & 0.660 & 0.297 & 0.464 & 0.474 \\
        
        \midrule
        \multicolumn{5}{c}{\bf{Pre-training \emph{w/o} Ontology Structure}} \\
        \midrule

        Geneformer & 0.616 & 0.261 & 0.418 & 0.432 \\
        scGPT & 0.615 & 0.258 & 0.442 & 0.438 \\
        scTab & \underline{0.707} & \underline{0.479} & 0.544 & \underline{0.577} \\
        UCE & 0.670 & 0.304 & 0.494 & 0.489 \\
        \mgprepro & 0.662 & 0.306 & 0.451 & 0.473 \\
        \suprepro & 0.703 & 0.393 & \underline{0.569} & 0.555 \\
        \mgpsuprepro & 0.661 & 0.337 & 0.550 & 0.516 \\

        \midrule
        \multicolumn{5}{c}{\bf{Pre-training \emph{w/} Ontology Structure}} \\
        \midrule
        
        \method & \bf{0.785} & \bf{0.558} & \bf{0.667} & \bf{0.670} \\
        
        \bottomrule
        \end{tabular}
    \end{adjustbox}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.56\textwidth}
    \centering
    \caption{Out-of-distribution Zero-shot Clustering ({\bf{AvgBio}$\uparrow$}). Other metrics are reported in App.~\ref{} due to space constraints.}
    %\label{tab:outdist_cell_type_clustering}
    %\footnotesize
    \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{l|cc|cc|cc|c}
        
        \toprule
        \multirow{2}{*}{\bf{Method}} & \multicolumn{2}{c|}{OOD CellType} & \multicolumn{2}{c|}{OOD Tissue } & \multicolumn{2}{c|}{OOD Donor } & \multirow{2}{*}{Average$\uparrow$} \\

        \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} 
        & $D^{ct}_{1}$ & $D^{ct}_{2}$ & $D^{ts}_{1}$ & $D^{ts}_{2}$ & $D^{dn}_{1}$ & $D^{dn}_{2}$ &\\

        \midrule

        \multicolumn{8}{c}{\bf{Traditional Methods \emph{w/o} Pre-training}} \\
        \midrule

        Raw Data & 0.703 & 0.629 & 0.540 & 0.631 & 0.458 & 0.460 & 0.570 \\
        Seurat & 0.752 & 0.737 & 0.587 & 0.636 & 0.466 & 0.489 & 0.611 \\
        Harmoney & 0.432 & 0.417  & 0.462  & 0.515 & 0.456 & 0.474  & 0.459 \\
        scVI & 0.760 & 0.725 & 0.577 & 0.634 & 0.478 & 0.502 & 0.613\\
        
        
        
        \midrule
        \multicolumn{8}{c}{\bf{Pre-training \emph{w/o} Ontology Structure}} \\
        \midrule

        Geneformer & 0.689   & 0.668   & 0.539 & 0.597  & 0.468 & 0.482 & 0.574 \\
        scGPT & 0.707   & 0.720    & 0.544 & 0.627    & 0.456     & 0.477 & 0.589 \\
        scTab & \underline{0.759} & 0.726 & 0.515 & 0.657 & OOM & OOM & / \\
        UCE & \bf{0.772} & 0.741 & 0.598 & 0.670 & 0.485 & 0.506 & 0.629 \\
        \mgprepro & 0.714 & 0.740 & 0.576 & 0.628  & 0.488 & 0.518   & 0.611 \\
        \suprepro & \bf{0.767} & \underline{0.775} & \underline{0.605}   & \underline{0.680} & 0.552 & \underline{0.573} & \underline{0.659} \\
        \mgpsuprepro & 0.758  & 0.764 & \bf{0.610} & 0.672 & \underline{0.553} & 0.570     & 0.655 \\
        
        
        
        \midrule
        \multicolumn{8}{c}{\bf{Pre-training \emph{w/} Ontology Structure}} \\
        \midrule

        \method & \bf{0.769} & \bf{0.786} & \bf{0.612} & \bf{0.705}  & \bf{0.608}  & \bf{0.643} & \bf{0.687} \\

        \bottomrule
        \end{tabular}
    \end{adjustbox}
    
    \end{minipage}
\end{table}

\fi

==> sections/figure_tex/_loss_ablation.tex <==
\begin{table}[t]
    \begin{minipage}[t]{0.65\textwidth}
        \centering
        \caption{\textbf{Pre-training Loss Ablation} on cell type clustering and novel cell type classification (\emph{abbr.}, "clf.").}
        %\label{tab:loss_ablation}
        \begin{adjustbox}{max width=\textwidth}
            \begin{tabular}{l|cc|cc}
                \toprule
                \multirow{3}{*}{\bf{Config}} & \multicolumn{2}{c|}{\textbf{Cell Type Clustering} } & \multicolumn{2}{c}{\textbf{Novel Cell Type Clf.}}  \\
                \cmidrule{2-5}
                & \multicolumn{1}{c}{$D^{ct}_2$ }& \multicolumn{1}{c|}{ $D^{dn}_2$ } & \multicolumn{2}{c}{ $D^{ct}_1$} \\
                \cmidrule{2-5}
                %& \multicolumn{1}{c}{avg\_bio$\uparrow$ }& \multicolumn{1}{c|}{avg\_bio$\uparrow$ } & \multicolumn{1}{c}{OOD Data \#1 }& \multicolumn{1}{c}{OOD Data \#1 }\\
                \cmidrule{2-5}
                & avg\_bio$\uparrow$ & avg\_bio$\uparrow$ & Acc$\uparrow$ & Macro F1$\uparrow$\\
                \midrule
    
                Full Loss & 0.786 & 0.643 & 0.335  & 0.150 \\
                \midrule
                
                \emph{w/o} ${\gL}_{\mathrm{MGP}}$ & 0.774 $_{(\downarrow 1.5\%)}$ & 0.640 $_{(\downarrow 0.5\%)}$ & 0.287 $_{(\downarrow 14.3\%)}$ & 0.131 $_{(\downarrow 12.7\%)}$ \\
                \emph{w/o} ${\gL}_{\mathrm{Inter}}$ & 0.778 $_{(\downarrow 1.0\%)}$ & 0.620 $_{(\downarrow \bf{3.6}\%)}$ & 0.147 $_{(\downarrow \bf{56.1}\%)}$  & 0.052 $_{(\downarrow \bf{65.3}\%)}$ \\
                \emph{w/o} ${\gL}_{\mathrm{Intra}}$ & 0.730 $_{(\downarrow \bf{7.1}\%)}$ & 0.626 $_{(\downarrow \underline{2.6}\%)}$ & 0.280 $_{(\downarrow \underline{16.4}\%)}$  & 0.118 $_{(\downarrow \underline{21.3}\%)}$ \\
                \emph{w/o} ${\gL}_{\mathrm{Reg}}$ & 0.764 $_{(\downarrow \underline{2.8}\%)}$ & 0.638 $_{(\downarrow 0.8\%)}$ & 0.296 $_{(\downarrow 11.6\%)}$  & 0.134 $_{(\downarrow 10.7\%)}$ \\
                \bottomrule
            \end{tabular}
        \end{adjustbox}
    \end{minipage}
    
    \vspace{-0.5cm}
\end{table}


==> sections/figure_tex/_marker_gene_prediction.tex <==
\begin{table}[t]
    \begin{minipage}[t]{0.35\textwidth}
    \centering
        \caption{\textbf{Marker Gene Prediction}. }
        %\vspace{1.em}
        %\label{tab:exp_marker_gene_prediction}
    \begin{adjustbox}{max width=0.89\textwidth}
        \begin{tabular}{l|cc}
            \toprule
                Method & $D_1^{mk}$ & $D_2^{mk}$ \\
            
            \midrule
            \multicolumn{3}{c}{\bf{Ontology-Agnostic TFMs}} \\
            \midrule
            
            Geneformer & 0.4524 & 0.470  \\
            scGPT & 0.3854 & 0.387 \\
            scTab & & \\
            UCE & & \\
            \mgprepro & 0.5788 & 0.629 \\
            \suprepro  & 0.6994 & \underline{0.693}  \\
            \mgpsuprepro & \underline{0.7302} & \bf{0.730}  \\
            % \method (240202_181731, not pass_cell_cls)  & \bf{0.760} & \bf{0.744} & \bf{0.759} & \bf{0.754}  & \bf{0.749}  & \bf{0.729} \\
            \midrule
            \multicolumn{3}{c}{\bf{Ontology-Enhanced TFMs}} \\
            \midrule
            \method  & \bf{0.7564} & \bf{0.729} \\
            
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \end{minipage}
\end{table}
